RelightVid: Temporal-Consistent Diffusion Model for Video Relighting

Diffusion models have demonstrated remarkable success in image generation and editing, with recent advancements enabling albedo-preserving image relighting. However, applying these models to video relighting remains challenging due to the lack of paired video relighting datasets and the high demands for output fidelity and temporal consistency, further complicated by the inherent randomness of diffusion models. To address these challenges, we introduce RelightVid, a flexible framework for video relighting that can accept background video, text prompts, or environment maps as relighting conditions. Trained on in-the-wild videos with carefully designed illumination augmentations and rendered videos under extreme dynamic lighting, RelightVid achieves arbitrary video relighting with high temporal consistency without intrinsic decomposition while preserving the illumination priors of its image backbone.

==> fig_tex/bg_sync_result.tex <==
\begin{figure*}[htbp]
\centering
\includegraphics[width=0.95\textwidth]{fig/long_result7.pdf}
\caption{\textbf{Synthetic background-condition illumination editing results.} We use the Hunyuan model for long synthetic background videos with strong dynamic lighting, demonstrating the effectiveness and robustness of our method in scenarios with dynamic lighting and long videos editing.}
\label{fig:bg_sync_result}
\vspace{-2mm}
\end{figure*}

==> sec/6_acks.tex <==
% DO NOT INCLUDE ACKNOWLEDGMENTS IN AN ANONYMOUS SUBMISSION TO SIGGRAPH 2019
\begin{acks}

This project is funded in part by Shanghai Artificial lntelligence Laboratory, the National Key R\&D Program of China (2022ZD0160201), the Centre for Perceptual and Interactive Intelligence (CPII) Ltd under the Innovation and Technology Commission (ITC)’s InnoHK.

\end{acks}
